On a Generalization of Wasserstein Distance and the Beckmann Problem to Connection Graphs

We propose a model of optimal parallel transport between vector fields on a connection graph, which consists of a weighted graph along with a map from its edges to an orthogonal group. Inspired by the well-known equivalence of 1-Wasserstein distance and minimum cost flows on standard graphs, we consider two versions of this problem: a minimum norm vector-valued flow problem with divergence constraints reflective of the connection structure of the graph; and a modified version which incorporates both quadratic regularization and a relaxation of the divergence constraint. Our theoretical contributions include: conditions for feasibility and computation of the Lagrangian dual problem for both problems, and duality correspondence for the relaxed-regularized version. Example applications of the model including transport between color images, vector field interpolation, and unsupervised clustering of vector field-valued data (in this case hurricane trajectory data) are also considered.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{amssymb,amsmath}
\usepackage{enumitem}
\usepackage{mathtools}
\usepackage{mathtools}
% \mathtoolsset{showonlyrefs}
\usepackage{autonum}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

\usepackage{caption}
\usepackage{subcaption}
\usepackage[normalem]{ulem}

\newcommand{\abs}[1]{|{#1}|}
\newcommand{\norm}[1]{||{#1}||}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Fi}{\mathbb{F}}
\newcommand{\ip}[1]{\langle {#1} \rangle}
\newcommand{\sr}{\mathcal{R}}
\newcommand{\prb}[1]{\mathbb{P}\left[{#1}\right]}
\newcommand{\ept}[1]{\mathbb{E}\left[{#1}\right]}
\newcommand{\lip}[1]{\operatorname{Lip_0}{(#1)}}
\newcommand{\brln}{\vspace{0.25cm}\\}
\newcommand{\lm}[1]{\mathcal{L}({#1})}
\newcommand{\Lm}[1]{L({#1})}
\newcommand{\supp}{{\text{supp}}}
\newcommand{\sgn}{{\text{sgn}}}
\newcommand{\room}{{\hspace{.2cm}}}
\newcommand{\Room}{{\hspace{.5cm}}}
\newcommand{\concat}[2]{{#1}{#2}} % old notation: \newcommand{\concat}[2]{{#1}+{#2}}

\usepackage{xcolor, soul}

\newcommand{\hlc}[2][yellow]{{%
    \colorlet{foo}{#1}%
    \sethlcolor{foo}\hl{#2}}%
}

\newcommand{\dhruv}[1] {{ \textcolor{red}{\hlc[red!15]{\sf [DK:] #1}}}}
\newcommand{\sawyer}[1] {{ \textcolor{blue}{\hlc[blue!15]{\sf [SJR:] #1}}}}
\newcommand{\gal}[1] {{ \textcolor{green}{\hlc[green!15]{\sf [GM:] #1}}}}
\newcommand{\alex}[1] {{ \textcolor{cyan}{\hlc[cyan!15]{\sf [AC:] #1}}}}

\newtheorem{example}{Example}[section]

\crefname{section}{Section}{Sections}
\crefname{subsection}{Subsection}{Subsections}
\crefname{align}{Eq.}{Eqs.}

\newcommand{\needcite}{{ \textcolor{red}{\hlc[yellow!50]{\sf [Citation needed]}}}}

% \newcommand{\old}[1] {{\textcolor{red}{\hlc[red!15]{#1}}}}
% \newcommand{\new}[1] {{\textcolor{black}{\hlc[blue!10]{#1}}}}
% \newcommand{\note}[1] {{\textcolor{black}{\hlc[yellow!50]{[[\sf \textbf{NOTE}: #1]]}}}}

% \newcommand{\new}[1]{{\color{blue}{#1}}}
% \newcommand{\old}[1]{{}}
% \newcommand{\note}[1] {{\textcolor{black}{\hlc[yellow!50]{[[\sf \textbf{NOTE}: #1]]}}}}

\newcommand{\note}[1] {{}}
\newcommand{\old}[1]{{\color{red!40}{}}}
\newcommand{\new}[1]{{#1}}

\usepackage{tikz}
\usepackage{tikz-3dplot} 
\usepackage{pgfplots, pgfplotstable}
\usetikzlibrary{3d} 
\usetikzlibrary{arrows.meta}


% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{The Beckmann Problem on Connection Graphs}{S. Robertson, D. Kohli, G. Mishne, A. Cloninger}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{On a Generalization of Wasserstein Distance and the Beckmann Problem to Connection Graphs}
%\thanks{submitted to editors DATE.}}

% Authors: full names plus addresses.
% \author{
% Sawyer Jack Robertson\thanks{Institute info \# 1} \and
% Dhruv Kohli\thanks{Institute info \# 2}
% }
\author{Sawyer Jack Robertson\footnotemark[4] \thanks{Department of Mathematics, UC San Diego (\url{s5robert@ucsd.edu}, \url{dhkohli@ucsd.edu}).} \and
Dhruv Kohli\footnotemark[4] \footnotemark[1] 
\and Gal Mishne\thanks{Halicio\u{g}lu Data Science Institute, UC San Diego 
  (\url{gmishne@ucsd.edu}, \url{acloninger@ucsd.edu}).}
\and Alexander Cloninger\footnotemark[1]\ \footnotemark[2]}


\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%% Added on Overleaf: enabling xr
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
%%% END HELPER CODE
%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

